On the Validity of Consensus

The Byzantine consensus problem involves $n$ processes, out of which t < n could be faulty and behave arbitrarily. Three properties characterize consensus: (1) termination, requiring correct (non-faulty) processes to eventually reach a decision, (2) agreement, preventing them from deciding different values, and (3) validity, precluding ``unreasonable'' decisions. But, what is a reasonable decision? Strong validity, a classical property, stipulates that, if all correct processes propose the same value, only that value can be decided. Weak validity, another established property, stipulates that, if all processes are correct and they propose the same value, that value must be decided. The space of possible validity properties is vast. However, their impact on consensus remains unclear. This paper addresses the question of which validity properties allow Byzantine consensus to be solvable with partial synchrony, and at what cost. First, we determine necessary and sufficient conditions for a validity property to make the consensus problem solvable; we say that such validity properties are solvable. Notably, we prove that, if n <= 3t, all solvable validity properties are trivial (there exists an always-admissible decision). Furthermore, we show that, with any non-trivial (and solvable) validity property, consensus requires Omega(t^2) messages. This extends the seminal Dolev-Reischuk bound, originally proven for strong validity, to all non-trivial validity properties. Lastly, we give a general Byzantine consensus algorithm, we call Universal, for any solvable (and non-trivial) validity property. Importantly, Universal incurs O(n^2) message complexity. Thus, together with our lower bound, Universal implies a fundamental result in partial synchrony: with t \in Omega(n), the message complexity of all (non-trivial) consensus variants is Theta(n^2).

==> sections/application.tex <==
\section{Our Results in the Wild}

In this section, we investigate some well-studied validity properties. 
Specifically, we study the consequences our findings yield when applied to specific validity properties.

\subsection{Our Results in the Context of Well-Studied Validity Properties}

\paragraph{Strong Validity}
Recall that \emph{Strong Validity}~\cite{CGL18,civit2022byzantine,Momose2021} states that, if all correct processes propose the same value, only that value can be decided.
Observe that \emph{Strong Validity} is a non-trivial validity property.
As such, due to \Cref{theorem:triviality_main}, \emph{Strong Validity} is unsolvable with $n \leq 3t$.

Moreover, Dolev-Reischuk bound states that \emph{Strong Validity} requires $\Omega(t^2)$ messages (and words) to be sent by correct processes.
When $O(t) = O(n)$, the bound is tight: Civit \emph{et al.}~\cite{civit2022byzantine} introduced \textsc{Squad}, a Byzantine consensus algorithm with \emph{Strong Validity}, which achieves $O(n^2)$ message and communication complexities.
In this paragraph, we show that the structure of \textsc{Squad} is similar to the structure of our general algorithm.

\textsc{Squad} is built on top of \textsc{Quad}.
The authors assume an existence of a $(n - 2t, n)$-threshold signature scheme~\cite{libert2014born}.
In a nutshell, these are the steps taken by a correct process $P_i$ in \textsc{Squad}:
\begin{compactenum}
    \item Process $P_i$ broadcasts its proposal $v \in \mathcal{V}_I$, which is share-signed by $P_i$ (with the threshold $n - 2t$).

    \item Once $P_i$ collects $n - t$ proposals, it checks whether there exists a proposal $v^*$ sent by (at least) $n - 2t$.
    
    \begin{compactenum}
        \item If there is, $P_i$ creates a constant-sized threshold signature $\sigma^*$ and proposes $(v^*, \sigma^*)$ to \textsc{Quad}.

        \item Otherwise:
        \begin{compactenum}
            \item $P_i$ broadcasts a predetermined string ``any value'', which is share-signed by $P_i$ (with the threshold $n - 2t$).

            \item $P_i$ waits to obtain either a ``positivity'' proof $\sigma_p$ for some value $v_p$ ($n - 2t$ identical proposals for $p$) or a ``negativity'' proof $\sigma_n$ ($n - 2t$ ``any value'' messages).
            Once this happens, $P_i$ either proposes (1) $(v_p, \sigma_p)$, or (2) $(\mathit{default\_value}, \sigma_n)$ to \textsc{Quad}.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}
Importantly, the pre-processing phase of \textsc{Squad} exists solely for ensuring that the proofs forwarded to \textsc{Quad} are of constant size.
Hence, the structure of \textsc{Squad} is similar to the structure of our general algorithm.
Indeed, our Byzantine consensus algorithm with \emph{Interactive-Consistency Validity} could be modified (in the same way as the pre-processing phase of \textsc{Squad}) to allow constant-sized proofs in the case of \emph{Strong Validity}.

\paragraph{Weak Validity}
\emph{Weak Validity} says that, if all processes are correct and propose the same value, only that value can be decided.
As \emph{Weak Validity} is non-trivial, it cannot be solved with $n \leq 3t$ (by \Cref{theorem:triviality_main}).
Note that \textsc{Quad}~\cite{civit2022byzantine}, a Byzantine consensus algorithm with \emph{Weak Validity}, achieves $O(n^2)$ message and communication complexities.
However, until now, it was not known what the lower bound on message and communication complexities was for Byzantine consensus algorithm with \emph{Weak Validity}.
As we show, the lower bound are $\Omega(t^2)$, which further proves that \textsc{Quad} is indeed optimal (as $t = O(n)$ in \textsc{Quad}).

\paragraph{From-Correct Validity}
Thus far, we have not mentioned \emph{From-Correct Validity}.
\begin{compactitem}
    \item \emph{From-Correct Validity:} If a correct process decides a value $v$, then $v$ was proposed by a correct process.
\end{compactitem}
This validity property was used to define the \emph{strong consensus} problem~\cite{fitzi2003efficient}.

In their paper~\cite{fitzi2003efficient}, Fitzi and Garay show that Byzantine consensus algorithm with \emph{From-Correct Validity} is exists if and only if $n > (|\mathcal{D}| + 1)t$, where $\mathcal{D} = |\mathcal{V}_I|$.
We now show the same result using our formalism.

\begin{theorem} [new proof]
Solving the Byzantine consensus problem with \emph{From-Correct Validity} is possible if and only if $n > (d + 1)t$, where $d = |\mathcal{V}_I| = |\mathcal{V}_O|$.
\end{theorem}
\begin{proof}
First, we show that, if $n \leq (d + 1)t$, it is impossible to solve the Byzantine consensus problem with \emph{From-Correct Validity}.
By contradiction, suppose that it is possible to solve the Byzantine consensus problem with \emph{From-Correct Validity} with $n \leq (d + 1)t$.
Let $\mathit{base} \in \mathcal{I}$ be an input configuration such that (1) $|\mathit{base}| = n - t$, and (2) no proposal $v \in \mathcal{V}_I$ appears with more than $t$ processes in $\mathit{base}$; note that we can construct $\mathit{base}$ as $n - t \leq dt$.
For every value $v \in \mathcal{V}_I$, we construct an input configuration $c_v \in \mathcal{I}$ in the following way:
\begin{compactenum}
    \item Let $c_v \gets \mathit{base}$.

    \item We remove from $c_v$ all process-proposal pairs $\mathit{pp}$ with $\mathsf{proposal}(\mathit{pp}) = v$.

    \item For every process $P \notin \processes{\mathit{base}}$, we add $(P, v')$ to $c_v$, where $v' \neq v$.
\end{compactenum}
For every input configuration $c_v$, (1) $c_v \sim \mathit{base}$, and (2) $\text{\emph{From-Correct Validity}}(c_v) = \mathcal{V}_O \setminus{\{v\}}$.
Hence, \emph{From-Correct Validity} does not satisfy $\mathcal{C}_S$, which contradicts \Cref{theorem:similarity_condition_necessary}.
Thus, it is impossible that $n \leq (d + 1)t$.
\end{proof}

\subsection{On External Validity}


==> sections/byzantine.tex <==
\section{Validity Properties in the Byzantine Failure Model}

In this section, we investigate the validity properties of the consensus problem in the Byzantine failure model.

\subsection{Preliminaries}

\paragraph{System model.}
We consider a static system $\Psi = \{P_1, ..., P_n\}$ of $n$ processes among which $f < n$ processes can be Byzantine.
If a process is Byzantine, the process is \emph{faulty}; otherwise, the process is \emph{correct}.

\paragraph{Byzantine consensus.}
Each process has its \emph{proposal}, and it should eventually \emph{decide}.
We denote by $\mathcal{V}$ the set of values a process can propose and decide.
The consensus problem in the Byzantine failure model requires the following three properties to hold:
\begin{compactitem}
    \item \emph{Agreement:} No two correct processes decide different values.
    
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Validity}
\end{compactitem}

\paragraph{Validity property.}
First, we define a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$ is a value.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.

Next, an \emph{input configuration} is a tuple $\big[ \mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_x \big]$, where (1) $\mathit{pp}_i$ is a process-proposal, for every $i \in [1, x]$, (2) $x \geq n - f$, and (3) every process-proposal pair is associated with a distinct process.
We denote by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$; if such process-proposal does not exist, $\mathit{input}[i] = \bot$.
% Furthermore, $\mathit{correct}(\mathit{input} \in \mathcal{I}) = \{P \,|\, (P, *) \text{ belongs to } \mathit{input}\}$ denotes the set of correct processes as established by $\mathit{input}$.
% Lastly, we define $\mathit{identical\_proposals}: \mathcal{I} \times \mathcal{I} \to \{\mathit{false}, \mathit{true}\}$ such that $\mathit{identical\_proposals}(i_1 \in \mathcal{I}, i_2 \in \mathcal{I}) = \top$ if and only if every process is associated with the same proposal in both $i_1$ and $i_2$.

By slightly abusing the notation, for any two input configurations $i_1, i_2 \in \mathcal{I}$, we define $i_1 \subseteq i_2$ in the following manner:
\begin{equation*}
    i_1 \subseteq i_2 \iff \forall j \in [1, n]: i_1[j] \neq \bot \implies i_2[j] = i_1[j].
\end{equation*}
In other words, $i_1 \subseteq i_2$ if and only if, the set that corresponds to the input configuration $i_1$ is a subset of the set that corresponds to the input configuration $i_2$.

We define a \emph{validity property} $\mathit{val}$ as a function $\mathcal{I} \to 2^{\mathcal{V}}$ such that, for every $\mathit{input} \in \mathcal{I}$, $\mathit{val}(\mathit{input}) \neq \emptyset$.
Finally, we say that a Byzantine consensus algorithm $\mathcal{A}_B$ satisfies a validity property $\mathit{val}$ if and only if the following holds:
\begin{compactitem}
    \item \emph{Validity safety:} In every execution $e$ of $\mathcal{A}_B$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.
    
    \item \emph{Validity liveness:} For every input configuration $\mathit{input} \in \mathcal{I}$ and every value $v \in \mathit{val}(\mathit{input})$, there exists an execution $e$ of $\mathcal{A}_B$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
\end{compactitem}

\subsection{Synchronous Environments}

First, we investigate validity properties of Byzantine consensus in a synchronous setting.

\paragraph{Communication.}
In a synchronous environment, there exists an upper bound $\Delta$ on message delays between processes.
In other words, if a correct process sends a message to another correct process at time $t$, the message will be received by time $t + \Delta$; note that the message might be received at time $t^* \in [t, t + \Delta]$ (the actual message delay for each message is chosen by the adversary).

\paragraph{Necessary conditions.}
We start by introducing the \emph{Byzantine containment condition}.

\begin{definition} [Byzantine containment condition] \label{definition:Byzantine_containment}
Let $\mathit{val}$ be a validity property.
We say that $\mathit{val}$ satisfies the \emph{Byzantine containment condition} if and only if the following holds:
\begin{equation*}
    \forall i_1, i_2 \in \mathcal{I}: i_1 \subseteq i_2 \implies \mathit{val}(i_2) \subseteq \mathit{val}(i_1).
\end{equation*}
\end{definition}

We now show that the Byzantine containment condition (\Cref{definition:Byzantine_containment}) is necessary for a validity property to be satisfiable in a Byzantine environment.

\begin{lemma} [Byzantine containment condition is necessary] \label{lemma:byzantine_containment_necessary}
Let $\mathit{val}$ be a validity property that does not satisfy the Byzantine containment condition.
No algorithm (even if synchronous) solves the Byzantine consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the Byzantine containment condition, there exist two input configuration $i_1, i_2 \in \mathcal{I}$ such that (1) $i_1 \subseteq i_2$, and (2) $\mathit{val}(i_2) \not\subseteq \mathit{val}(i_1)$.
In other words, there exists a value $x \in \mathcal{V}$ such that $x \in \mathit{val}(i_2)$ and $x \notin \mathit{val}(i_1)$.

By contradiction, suppose that there exists a Byzantine algorithm $\mathcal{A}_B$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_B$ be a synchronous algorithm.

Since $\mathcal{A}_B$ satisfies $\mathit{val}$, there exists an execution $e$ of $\mathcal{A}_B$ that corresponds to the input configuration $i_2$ in which the decided value is $x$ (due to the validity liveness).
We now create an execution $e'$ such that (1) $e'$ corresponds to $i_1$, and (2) the decided value in $e'$ is $x \notin \mathit{val}(i_1)$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item After the first correct process decides in $e'$, we crash all processes which are correct according to $i_2$ and faulty according to $i_1$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $x \notin \mathit{val}(i_1)$, which means that $\mathcal{A}_B$ does not satisfy $\mathit{val}$ in $e'$.
This contradicts the fact that $\mathcal{A}_B$ satisfies $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
We now show that the Byzantine containment condition is sufficient for a validity property to be satisfiable in a Byzantine setting.

\begin{theorem} [Byzantine containment condition is sufficient]
Let $\mathit{val}$ be a validity property that satisfies the Byzantine containment condition.
There exists an algorithm that solves the Byzantine consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a synchronous Byzantine-tolerant algorithm $\mathcal{A}_B$ that solves $\mathit{val}$.

Before devising $\mathcal{A}_B$, we are implementing a synchronous Byzantine-tolerant consensus algorithm $\mathcal{A}_{\mathit{correct}}$ in which processes agree on an input configuration.
Specifically, $\mathcal{A}_{\mathit{correct}}$ satisfies the following validity property:
\begin{compactitem}
    \item \emph{All-correct validity:} Let the decided value be $i = \big[ (P_{i_1}, v_{i_1}), (P_{i_2}, v_{i_2}), ..., (P_{i_x}, v_{i_x}) \big]$.
    Then, for every correct process $P_x$, $(P_x, v_x)$ belongs to $i$, where $v_x$ is the proposed value by $P_x$.
\end{compactitem}
Intuitively, $\mathcal{A}_{\mathit{correct}}$ allows correct processes to agree on the input configuration that contains \emph{all} process-proposals associated with correct processes.

\begin{algorithm}
\caption{Byzantine-tolerant algorithm $\mathcal{A}_{\mathit{correct}}$ that solves consensus with all-correct validity: Pseudocode for process $P_i$}
\label{algorithm:a_correct}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Byzantine Reliable Broadcast, \textbf{instance} $\mathit{brb}$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{trigger} $\langle \mathit{brb}, \mathsf{broadcast}([\textsc{proposal}, \mathit{proposal}]) \rangle$

\medskip
\LineComment{$\mathit{brb}$ is implemented using synchronous HotStuff protocol accompanied by the certification phase given in the DISC submission}
\State \textbf{At time $8(f + 1)\Delta + 3\Delta$:} \label{line:decide_all_correct}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\text{the input configuration built out of all delivered \textsc{proposal} messages})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_{\mathit{correct}}$ (\Cref{algorithm:a_correct}) solves the Byzantine consensus problem with all-correct validity:
\begin{compactitem}
    \item Termination: Termination holds as every correct process decides at time $8(f + 1)\Delta + 3\Delta$ (line~\ref{line:decide_all_correct}).
    
    \item Agreement: Agreement follows from the agreement property of $\mathit{brb}$ and the fact that, if a correct process delivers a message from $\mathit{brb}$, it does so by time $8(f + 1)\Delta + 3\Delta$.
    
    \item All-correct validity: Follows from the validity property of $\mathit{brb}$ and the fact that a message $\mathit{brb}$-broadcast by a correct process is $\mathit{brb}$-delivered by time $8(f + 1)\Delta + 3\Delta$.
\end{compactitem}

Finally, we are ready to present $\mathcal{A}_B$.

\begin{algorithm}
\caption{Byzantine-tolerant algorithm $\mathcal{A}_B$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:synchronous_byzantine}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Byzantine-Tolerant Consensus with All-Correct Validity, \textbf{instance} $\mathcal{A}_{\mathit{correct}}$
\State \hskip2em Synchronous Byzantine-Tolerant Consensu with External Validity, \textbf{instance} $c$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{trigger} $\langle \mathcal{A}_{\mathit{correct}}, \mathsf{propose}(\mathit{proposal}) \rangle$

\medskip
\State \textbf{upon} $\langle \mathcal{A}_{\mathit{correct}}, \mathsf{decide}(i) \rangle$:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \text{a value from } \mathit{val}(i)$
\State \hskip2em \(\triangleright\) values which are valid for $c$ are all the values from $\mathit{val}(i)$
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$
\end{algorithmic}
\end{algorithm}

Termination of $\mathcal{A}_B$ follows from termination of $\mathcal{A}_{\mathit{correct}}$ and $c$.
Furthermore, agreement of $\mathcal{A}_B$ follows from agreement of $c$.
Hence, we need to prove the validity property of $\mathcal{A}_B$.

Fix an input configuration $\mathit{input}$.
Since all correct processes agree in $\mathcal{A}_{\mathit{correct}}$ on an input configuration $i$, all correct processes agree on the set of valid values in $c$.
Hence, the decided value $v \in \mathit{val}(i)$.
Moreover, we have that $\mathit{input} \subseteq i$ (due to the all-correct validity of $\mathcal{A}_{\mathit{correct}}$).
Thus, $v \in \mathit{val}(\mathit{input})$ (since $\mathit{val}$ satisfies the Byzantine containment condition), and the validity safety property is ensured.

As for the validity liveness, we can easily modify $\mathcal{A}_{\mathit{correct}}$ to take into account the exact time of decision.
Then, as done before, we can map the time into a specific value from $\mathit{val}(i)$.
Therefore, validity liveness is (i.e., can be) ensured by $\mathcal{A}_B$, which concludes the theorem.
\end{proof}

\subsection{Partially Synchronous Environments}

Next, we investigate validity properties of Byzantine consensus in a partially synchronous setting.

\paragraph{Communication.}
In a partially synchronous environment, there exists an unknown time Global Stabilization Time (GST) such that the system behaves asynchronously before GST, and behaves synchronously after GST.
Formally, there exist a known upper bound $\delta$ on message delays after GST.

\paragraph{Necessary conditions.}
First, note that the Byzantine containment condition is necessary for a validity property to be satisfied in a partially synchronous environment (as this condition is necessary in a synchronous setting).
We now define when an input configuration is ``Byzantine-correct-similar'' to another configuration.
Formally, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{ByzSim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{ByzSim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j] \neq \bot \land i'[j] \neq \bot \implies \mathit{input}[j] = i'[j]\}.
\end{equation*}
In other words, an input configuration $i' \in \mathcal{I}$ is \emph{Byzantine-correct-similar} to $\mathit{input}$ if all processes which belong to both $\mathit{input}$ and $i'$ propose the same values in both input configurations.

Next, we introduce the \emph{Byzantine-correct-similarity condition}.

\begin{definition} [Byzantine-correct-similarity condition] \label{definition:f+1_similarity}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{AlmostSim}(\mathit{input}) = \{\mathit{input}' \in \mathcal{I} \,|\, \text{proposed values of processes correct according to } i \text{ are identical}\}$.
We say that $\mathit{val}$ satisfies the \emph{Byzantine-correct-similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{ByzSim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

We now show that the Byzantine-correct-similarity condition is necessary in a partially synchronous setting.

\begin{lemma} [Byzantine-correct-similarity condition is necessary] \label{lemma:f+1_similarity_necessary}
Let $\mathit{val}$ be a validity property that does not satisfy the Byzantine-correct-similarity condition.
No partially synchronous algorithm solves the Byzantine consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the Byzantine-correct-similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{ByzSim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:f+1_similarity}).
By contradiction, suppose that there exists a partially synchronous Byzantine consensus algorithm $\mathcal{A}_B$ that satisfies $\mathit{val}$.

Consider an execution $e$ of $\mathcal{A}_B$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); observe that there might be no faulty processes in $e$ (according to $i$).
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{ByzSim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the Byzantine-correct-similarity condition would be satisfied for $i$).

Now, we create an execution $e'$ of $\mathcal{A}_B$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item No process correct in both $e$ and $e'$ (there exist at least $f + 1$ such processes) hears from any process $P \in \Psi$ in $e'$ until a value is decided in $e'$, where $P$ is faulty in $e$ (i.e., according to $i$) and correct in $e'$ (i.e., correct according to $i'$).
    
    \item After a decision has been made in $e'$, we crash all processes which are faulty according to $i'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_B$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_B$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
Finally, we are ready to show that Byzantine containment and Byzantine-correct-similarity conditions are sufficient for a validity property to be satisfiable in a partially synchronous setting.

\begin{theorem} [Byzantine containment and Byzantine-correct-similarity conditions are sufficient in partial synchrony]
Let $\mathit{val}$ be a validity property that satisfies Byzantine containment and Byzantine-correct-similarity conditions.
There exists a partially synchronous algorithm that solves the Byzantine consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a partially synchronous Byzantine consensus algorithm $\mathcal{A}_B$ (\Cref{algorithm:partially_synchronous_byzantine}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Partially synchronous Byzantine algorithm $\mathcal{A}_B$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:partially_synchronous_byzantine}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Partially Synchronous Byzantine Consensus with External Validity, \textbf{instance} $c$
\State \hskip2em Byzantine Consistent Broadcast, \textbf{instance} $\mathit{bcb}$

\medskip
\State \textbf{upon} $\mathsf{start}$:
\State \hskip2em \textbf{trigger} $\langle \mathit{bcb}, \mathsf{broadcast}\big([\textsc{proposal}, \mathit{proposal}]\big) \rangle$

\medskip
\State \textbf{upon} delivery of $n - f$ \textsc{proposal} messages:
\State \hskip2em \textbf{trigger} timer for $\Delta$ time \Comment{$\Delta$ is some predefined constant}

\medskip
\State \textbf{upon} timer elapsed:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:partially_build_i_byzantine}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{ByzSim}(i)$ \label{line:partially_set_to_propose}

\State \hskip2em \(\triangleright\) all values are associated with received \textsc{proposal} messages which proves the validity of the proposed values
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:partially_propose_c_byzantine}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_B$ (\Cref{algorithm:partially_synchronous_byzantine}) solves the Byzantine consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a used partially synchronous Byzantine consensus (instance $c$ in \Cref{algorithm:partially_synchronous_byzantine}).
Hence, it is left to show that $\mathcal{A}_B$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_B$ satisfies the validity safety.
Let $P$ be a process that proposes to $c$ (at line~\ref{line:partially_propose_c_byzantine}) and let $i$ be the input configuration that corresponds to messages $P$ accompanies its proposal by.
We have the following: $i \in \mathit{ByzSim}(\mathit{input})$.
% ; observe that, if $P$ does not receive \textsc{proposal} messages from all processes, $i$ is not, strictly speaking, an input configuration.
% We ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not received a \textsc{proposal} message, we add $(\bar{P}', \text{any value})$ to $i$.
% Importantly, $\mathit{input} \in \mathit{CorrectSim}(i)$.
Hence, the proposed value must belong to $\mathit{val}(\mathit{input})$.
% Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Therefore, for every value $v$ proposed to the black-box partially synchronous Byzantine consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only values accompanied with \textsc{proposal} messages, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:partially_synchronous_byzantine}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_B$ relies on time.
We assume that the time maps to a value in the same way at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All correct processes propose their values according to $\mathit{input}$.
    All Byzantine processes immediately announce themselves by broadcasting ``I am Byzantine'' to all processes.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Every correct process receives messages from all correct processes before proposing to $c$.
\end{compactenum}
Hence, all correct processes build $\mathit{input}$ at line~\ref{line:partially_build_i_byzantine}.
Thus, all processes propose $v$ to $c$, which means $v$ is decided.
Let us underline that, in this case, the attack exploited in \Cref{lemma:f+1_similarity_necessary} cannot be used, which means that the execution preserves the safety violation (since $\mathit{val}$ satisfies the Byzantine containment property).
The theorem holds.
\end{proof}

==> sections/crash-stop.tex <==
\section{Validity Properties In The Crash-Stop Failure Model}

In this section, we take a closer look at the validity properties of the consensus problem in the crash-stop failure model.

\subsection{Preliminaries}

\paragraph{System model.}
We consider a static system $\Psi = \{P_1, ..., P_n\}$ of $n$ processes among which $f < n$ processes can fail by \emph{crashing}.
If a process crashes, the process is \emph{faulty}; otherwise, the process is \emph{correct}.
This failure model is known as the \emph{crash-stop} failure model.

\paragraph{Crash-stop consensus.}
Each process has its \emph{proposal}, and it should eventually \emph{decide}.
We denote by $\mathcal{V}$ the set of values a process can propose and decide.
The consensus problem in the crash-stop failure model requires the following three properties to hold:
\begin{compactitem}
    \item \emph{Agreement:} No two processes decide different values.
    
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Validity}
\end{compactitem}

\paragraph{Validity property.}
First, we define a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x$ is either $P \in \Psi$ or $\bar{P}$, with $P \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$ is a value.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$; on the other hand, $(\bar{P}, \mathit{val}')$ denotes that a \emph{faulty} process $P \in \Psi$ has proposed a value $\mathit{val}' \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.
Finally, $\mathit{pp}.\mathsf{correct}$ returns $\top$ if and only if $\mathit{pp}$ is associated with a correct processes; $\mathit{pp}.\mathsf{correct}$ returns $\bot$ otherwise.

Next, an \emph{input configuration} is a tuple $\big[ \mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_n \big]$, where (1) $\mathit{pp}_i$ is a process-proposal, for every $i \in [1, n]$, (2) every process-proposal pair is associated with a distinct process, and (3) at most $f$ process-proposals refer to faulty processes (i.e., there can exist at most $f$ process-proposals of the format $(\bar{P}, v)$, where $P \in \Psi$ and $v \in \mathcal{V}$).
We denote by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$.

Furthermore, $\mathit{correct}(\mathit{input} \in \mathcal{I}) = \{P \in \Psi \,|\, \mathit{pp} \text{ belongs to } \mathit{input} \land \mathit{pp}.\mathsf{process} = P \land \mathit{pp}.\mathsf{correct} = \top\}$ denotes the set of correct processes as established by $\mathit{input}$.
We define $\mathit{identical\_proposals}: \mathcal{I} \times \mathcal{I} \to \{\top, \bot\}$ in the following manner:
\begin{equation*}
    \mathit{identical\_proposals}(i_1, i_2) = \top \iff \forall j \in [1, n]: i_1[j].\mathsf{proposal} = i_2[j].\mathsf{proposal}.
\end{equation*}

We define a \emph{validity property} $\mathit{val}$ as a function $\mathcal{I} \to 2^{\mathcal{V}}$ such that, for every $\mathit{input} \in \mathcal{I}$, $\mathit{val}(\mathit{input}) \neq \emptyset$.
Finally, we say that a crash-stop consensus algorithm $\mathcal{A}_C$ satisfies a validity property $\mathit{val}$ if and only if the following holds:
\begin{compactitem}
    \item \emph{Validity safety:} In every execution $e$ of $\mathcal{A}_C$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.
    
    \item \emph{Validity liveness:} For every input configuration $\mathit{input} \in \mathcal{I}$ and every value $v \in \mathit{val}(\mathit{input})$, there exists an execution $e$ of $\mathcal{A}_C$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
\end{compactitem}


% Finally, we say that a crash-stop consensus algorithm $\mathcal{A}_C$ satisfies a validity property $\mathit{val}$ if and only if, in every execution $e$ of $\mathcal{A}_C$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.

% \paragraph{Core valid values.}
% Consider a crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies a validity property $\mathit{val}$.
% Let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
% We say that a value $v \in \mathit{val}(\mathit{input})$ is a \emph{core valid value} of $\mathit{input}$ in $\mathcal{A}_C$ if and only if there exists an execution $e$ of $\mathcal{A}_C$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
% We denote by $\mathit{core}(\mathcal{A}_C, \mathit{input})$ the set of core valid values of $\mathit{input}$ in $\mathcal{A}_C$; note that $\mathit{core}(\mathcal{A}_C, \mathit{input}) \subseteq \mathit{val}(\mathit{input})$.

% Why do we define core valid values?
% Consider an input configuration $\mathit{input} \in \mathcal{I}$.
% Since $\mathcal{A}_C$ satisfies $\mathit{val}$, $\mathcal{A}_C$ satisfies $\mathit{val}'$, which is a validity property identical to $\mathit{val}$, except that $\mathit{val}'(\mathit{input}) = \mathit{val}(\mathit{input}) \cup \{v^*\}$, where $v^* \notin \mathit{val}(\mathit{input})$.
% Indeed, $\mathcal{A}_C$ satisfies $\mathit{val}'$; however, $\mathcal{A}_C$ never decides $v^*$ in an execution that corresponds to $\mathit{input}$.
% Therefore, $v^*$ is not ``important'' to $\mathcal{A}_C$; we say that $v^*$ is \emph{not} a core valid value of $\mathit{input}$ in $\mathcal{A}_C$.
% In the rest of the section, we will usually talk about validity properties from the lenses of their core valid values.
 
\subsection{Synchronous Environments}

First, we investigate validity properties of crash-stop consensus in a synchronous setting.

\paragraph{Communication.}
In a synchronous environment, there exists an upper bound $\Delta$ on message delays between processes.
In other words, if a correct process sends a message to another correct process at time $t$, the message will be received by time $t + \Delta$; note that the message might be received at time $t^* \in [t, t + \Delta]$ (the actual message delay for each message is chosen by the adversary).

\paragraph{Necessary conditions.}
First, we define when two input configurations are similar.
Specifically, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{Sim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{Sim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j].\mathsf{correct} = \top \lor \mathit{i'}[j].\mathsf{correct} = \top \implies \mathit{input}[j] = \mathit{i'}[j]\}.
\end{equation*}
In other words, $i' \in \mathit{Sim}(\mathit{input})$ if and only if both input configurations have the identical ``set'' of process-proposals concerned with correct processes.
Note that $\mathit{Sim}(\mathit{input}) = \{\mathit{input}\}$ if, for every $j \in [1, n]$, $\mathit{input}[j].\mathsf{correct} = \top$.
Next, we introduce the \emph{similarity condition}.

\begin{definition} [Similarity condition] \label{definition:similarity_crash}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{Sim}(\mathit{input}) = \{\mathit{input'} \in \mathcal{I} \,|\, \text{all process-proposals concerned with correct processes are identical in } \mathit{input} \text{ and } \mathit{input}'\}$.
We say that $\mathit{val}$ satisfies the \emph{similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{Sim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

Now, we show that crash-stop consensus with a validity property that does not satisfy the similarity condition (\Cref{definition:similarity_crash}) cannot be satisfied by any algorithm.

\begin{lemma} [Similarity condition is necessary] \label{lemma:similarity_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the similarity condition.
No algorithm (even if synchronous) solves the crash-stop consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{Sim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:similarity_crash}).
Note that $i$ does not contain only process-proposals concerned with correct processes; otherwise, $\bigcap\limits_{i' \in \mathit{Sim}(i)} \neq \emptyset$ as $\mathit{Sim}(i) = \{i\}$.
By contradiction, suppose that there exists a crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_C$ be a synchronous algorithm.

Consider an execution $e$ of $\mathcal{A}_C$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); recall that there are faulty processes in $e$ as $i$ does not contain only process-proposals concerned with correct processes.
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{Sim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the similarity condition would be satisfied for $i$).
Again, note that there exist some faulty processes according to $i'$ (since there exist faulty processes according to $i$).

Now, we create an execution $e'$ of $\mathcal{A}_C$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item For each process who is faulty according to $e'$ (and $e$), we set its proposed value according to $e'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_C$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_C$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

Next, we define the \emph{containment condition}.

\begin{definition} [Containment condition] \label{definition:containment_crash}
Let $\mathit{val}$ be a validity property.
% and let $\mathcal{A}_C$ be an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
We say that $\mathit{val}$ satisfies the \emph{containment condition} if and only if the following holds:
\begin{equation*}
    \forall i_1, i_2 \in \mathcal{I}: \big(\mathit{identical\_proposals}(i_1, i_2) = \top \land \mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)\big) \implies \mathit{val}(i_2) \subseteq \mathit{val}(i_1).
\end{equation*}
% \begin{equation*}
%     \forall i_1, i_2 \in \mathcal{I}: \big(\mathit{identical\_proposals}(i_1, i_2) = \top \land \mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)\big) \implies \mathit{core}(\mathcal{A}_C, i_2) \subseteq \mathit{val}(i_1).
% \end{equation*}
\end{definition}

Next, we show that the containment condition is necessary for a validity property to be ``satisfiable''.

\begin{lemma} [Containment condition is necessary] \label{lemma:containment_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the containment condition.
No algorithm (even if synchronous) solves the crash-stop consensus problem with $\mathit{val}$.
% Let $\mathit{val}$ be a validity property and let $\mathcal{A}_C$ be an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
% Then, $\mathit{val}$ satisfies the containment condition with respect to $\mathcal{A}_C$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the containment condition, there exist two input configurations $i_1, i_2 \in \mathcal{I}$ such that (1) $\mathit{identical\_proposals}(i_1, i_2) = \top$, (2) $\mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)$, and (3) $\mathit{val}(i_2) \not\subseteq \mathit{val}(i_1)$.
In other words, there exists a value $x \in \mathcal{V}$ such that $x \in \mathit{val}(i_2)$ and $x \notin \mathit{val}(i_1)$.

By contradiction, suppose that there exists a crash-stop algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_C$ be a synchronous algorithm.

Since $\mathcal{A}_C$ satisfies $\mathit{val}$, there exists an execution $e$ of $\mathcal{A}_C$ that corresponds to the input configuration $i_2$ in which the decided value is $x$ (due to the validity liveness).
We now create an execution $e'$ such that (1) $e'$ corresponds to $i_1$, and (2) the decided value in $e'$ is $x \notin \mathit{val}(i_1)$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item After the first process decides in $e'$, we crash all processes which are correct according to $i_2$ and faulty according to $i_1$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $x \notin \mathit{val}(i_1)$, which means that $\mathcal{A}_C$ does not satisfy $\mathit{val}$ in $e'$.
This contradicts the fact that $\mathcal{A}_C$ satisfies $\mathit{val}$, which concludes the lemma.
\end{proof}

% Hence, the similarity and containment conditions are necessary for a validity property to be ``satisfiable''.

% \begin{corollary}
% Let $\mathit{val}$ be a validity property for which there exists an algorithm $\mathcal{A}_C$ which solves the crash-stop consensus problem with $\mathit{val}$.
% Then, $\mathit{val}$ satisfies both similarity and containment conditions.
% % Then, $\mathit{val}$ satisfies both (1) the similarity condition, and (2) the containment condition with respect to $\mathcal{A}_C$.
% \end{corollary}

\paragraph{Sufficient conditions.}
We now show that the similarity and containment conditions are sufficient for a validity property to be satisfiable.

\begin{theorem} [Similarity and containment conditions are sufficient]
Let $\mathit{val}$ be a validity property that satisfies the similarity and the containment conditions.
There exists an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a synchronous crash-stop consensus algorithm $\mathcal{A}_C$ (\Cref{algorithm:synchronous_crash_stop}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Crash-stop algorithm $\mathcal{A}_C$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:synchronous_crash_stop}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Crash-Stop Consensus, \textbf{instance} $c$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{broadcast} $[\textsc{proposal}, \mathit{proposal}]$

\medskip
\State \textbf{At time $\Delta$:}
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:build_i}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{Sim}(i)$ \label{line:set_to_propose}
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:propose_c}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_C$ (\Cref{algorithm:synchronous_crash_stop}) solves the consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a black-box synchronous crash-stop consensus (instance $c$ in \Cref{algorithm:synchronous_crash_stop}).
Hence, it is left to show that $\mathcal{A}_C$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_C$ satisfies the validity safety.
Let $P \in \Psi$ be a process that proposes to $c$ (at line~\ref{line:propose_c}) and let $i$ be the ``input configuration'' $P$ constructs at line~\ref{line:build_i} (if $P$ does not hear from all processes, $i$ is not, technically speaking, an input configuration as it does not contain $n$ process-proposals).
We separate two cases:
\begin{compactitem}
    \item $P$ receives \textsc{proposal} messages from all processes:
    In this case, we have that $\mathit{identical\_proposals}(i, \mathit{input}) = \top$.
    Moreover, $\mathit{correct}(\mathit{input}) \subseteq \mathit{correct}(i)$.
    Since $\mathit{to\_propose} \in \mathit{val}(i)$, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$ (as $\mathit{val}$ satisfies the containment property). 
    Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$ in this case.
    
    \item $P$ does not receive \textsc{proposal} messages from all processes:
    In this case, $i$ does not contain proposals from all $n$ processes (i.e., $i$ is not, strictly speaking, an input configuration).
    Let $i^*$ be an input configuration identical to $i$, except that, for all processes whose proposal is missing in $i$, we add the process-proposal established by $\mathit{input}$; observe that all processes whose proposal is missing in $i$ are faulty according to $\mathit{input}$.
    
    Now, we ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not heard, we add $(\bar{P'}, \text{any value})$ to $i$.
    Observe that $i^* \in \mathit{Sim}(i)$.
    
    Let $\mathit{to\_propose} = v$ (set at line~\ref{line:set_to_propose}).
    Hence, $v \in \mathit{val}(i^*)$ (as $i^* \in \mathit{Sim}(i)$).
    
    Furthermore, we have that $\mathit{identical\_proposals}(i^*, \mathit{input}) = \top$ and $\mathit{correct}(\mathit{input}) \subseteq \mathit{correct}(i^*)$.
    According to the containment condition, $v \in \mathit{val}(\mathit{input})$.
\end{compactitem}
In both possible cases, we have that $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Hence, for every value $v$ proposed to the black-box synchronous consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only proposed values, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:synchronous_crash_stop}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_C$ relies on time (importantly, $\mathcal{A}_C$ can avoid relying on time if $|\mathit{val}(\mathit{input})| < \infty$, for every $\mathit{input} \in \mathcal{I}$; we leave this modification for the future work).
We assume that the function mapping time to values is the same at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All processes propose their values according to $\mathit{input}$.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Once all processes have decided from $c$, all processes faulty according to $\mathit{input}$ crash.
\end{compactenum}
Since all processes receive the first \textsc{proposal} message at the same time (which maps to $v$), all processes propose $v$ to $c$.
Hence, the decided value must be $v$ (due to the validity property of $c$).
The validity liveness property is satisfied, which concludes the theorem.
\end{proof}

\subsection{Partially Synchronous Environments}

Next, we investigate validity properties of crash-stop consensus in a partially synchronous setting.

\paragraph{Communication.}
In a partially synchronous environment, there exists an unknown time Global Stabilization Time (GST) such that the system behaves asynchronously before GST, and behaves synchronously after GST.
Formally, there exist a known upper bound $\delta$ on message delays after GST.

\paragraph{Necessary conditions.}
First, note that the similarity and containment conditions are necessary for a validity property to be satisfied in a partially synchronous environment (as these conditions are necessary in a synchronous setting).
We now define when an input configuration is ``correct-similar'' to another configuration.
Formally, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{CorrectSim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{CorrectSim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j].\mathsf{correct} = \top \implies \mathit{input}[j].\mathsf{proposal} = i'[j].\mathsf{proposal}\}.
\end{equation*}
In other words, an input configuration $i' \in \mathcal{I}$ is \emph{correct-similar} to $\mathit{input}$ if proposed values of processes correct according to $\mathit{input}$ are identical in $i'$ and $\mathit{input}$.

Observe that $i_1 \in \mathit{CorrectSim}(i_2)$ does not imply $i_2 \in \mathit{CorrectSim}(i_1)$.
For example, let $i_1 = \big[(P_1, v_1), (P_2, v_2), (\bar{P}_3, v_3)\big]$ and $i_2 = \big[(\bar{P}_1, v_1), (P_2, v_2), (P_3, v_3')\big]$.
We have that $i_2 \in \mathit{CorrectSim}(i_1)$, but $i_1 \notin \mathit{CorrectSim}(i_2)$.
Next, we introduce the \emph{correct-similarity condition}.

\begin{definition} [Correct-similarity condition] \label{definition:correct_similarity}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{AlmostSim}(\mathit{input}) = \{\mathit{input}' \in \mathcal{I} \,|\, \text{proposed values of processes correct according to } i \text{ are identical}\}$.
We say that $\mathit{val}$ satisfies the \emph{correct-similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{CorrectSim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

% Note that, if all processes are correct according to $i \in \mathcal{I}$, $\mathit{AlmostSim}(i)$ contains input configurations $i' \in \mathcal{I}$ such that $\mathit{identical\_proposals}(i, i') = \top$ and $\mathit{correct}(i') \subseteq \mathit{correct}(i)$.
We now show that the correct-similarity condition is necessary in a partially synchronous setting.

\begin{lemma} [Correct-similarity condition is necessary] \label{lemma:correct_similarity_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the correct-similarity condition.
No partially synchronous algorithm solves the crash-stop consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the correct-similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{CorrectSim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:correct_similarity}).
By contradiction, suppose that there exists a partially synchronous crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.

Consider an execution $e$ of $\mathcal{A}_C$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); observe that there might be no faulty processes in $e$ (according to $i$).
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{CorrectSim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the correct-similarity condition would be satisfied for $i$).

Now, we create an execution $e'$ of $\mathcal{A}_C$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    We adjust the proposals according to $i'$.
    
    \item No process correct in $e$ hears from any process $P \in \Psi$ in $e'$ until a value is decided in $e'$, where $P$ is faulty in $e$ (i.e., according to $i$) and correct in $e'$ (i.e., correct according to $i'$).
    
    \item After a decision has been made in $e'$, we crash all processes which are faulty according to $i'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_C$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_C$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
Finally, we are ready to show that similarity, containment and correct-similarity conditions are sufficient for a validity property to be satisfiable in a partially synchronous setting.

\begin{theorem} [Similarity, containment and correct-similarity conditions are sufficient in partial synchrony]
Let $\mathit{val}$ be a validity property that satisfies similarity, containment and correct-similarity conditions.
There exists a partially synchronous algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a partially synchronous crash-stop consensus algorithm $\mathcal{A}_C$ (\Cref{algorithm:partially_synchronous_crash_stop}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Partially synchronous crash-stop algorithm $\mathcal{A}_C$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:partially_synchronous_crash_stop}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Partially Synchronous Crash-Stop Consensus, \textbf{instance} $c$

\medskip
\State \textbf{upon} $\mathsf{start}$:
\State \hskip2em \textbf{broadcast} $[\textsc{proposal}, \mathit{proposal}]$

\medskip
\State \textbf{upon} reception of $n - f$ \textsc{proposal} messages:
\State \hskip2em \textbf{trigger} timer for $\Delta$ time \Comment{$\Delta$ is some predefined constant}

\medskip
\State \textbf{upon} timer elapsed:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:partially_build_i}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{CorrectSim}(i)$ \label{line:partially_set_to_propose}
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:partially_propose_c}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_C$ (\Cref{algorithm:partially_synchronous_crash_stop}) solves the consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a used partially synchronous crash-stop consensus (instance $c$ in \Cref{algorithm:partially_synchronous_crash_stop}).
Hence, it is left to show that $\mathcal{A}_C$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_C$ satisfies the validity safety.
Let $P$ be a process that proposes to $c$ (at line~\ref{line:partially_propose_c}) and let $i$ be the input configuration $P$ constructs at line~\ref{line:partially_build_i}; observe that, if $P$ does not receive \textsc{proposal} messages from all processes, $i$ is not, strictly speaking, an input configuration.
We ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not received a \textsc{proposal} message, we add $(\bar{P}', \text{any value})$ to $i$.
Importantly, $\mathit{input} \in \mathit{CorrectSim}(i)$.
Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Therefore, for every value $v$ proposed to the black-box partially synchronous consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only proposed values, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:partially_synchronous_crash_stop}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_C$ relies on time (importantly, $\mathcal{A}_C$ can avoid relying on time if $|\mathit{val}(\mathit{input})| < \infty$, for every $\mathit{input} \in \mathcal{I}$).
We assume that the time maps to a value in the same way at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All processes propose their values according to $\mathit{input}$.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Once all processes have decided from $c$, all faulty processes crash.
\end{compactenum}
Since all processes receive the first \textsc{proposal} message at the same time (which maps to $v$), all processes propose $v$ to $c$.
Hence, the decided value must be $v$ (due to the validity property of $c$).
The theorem holds. 
\end{proof}

==> sections/crash.tex <==
\section{Validity Properties of the Crash-Stop Consensus}

In this section, we deal with the satisfiability of the validity properties of the crash-stop consensus problem.
First, we formally define a validity property of the crash-stop consensus (\Cref{subsection:crash_stop_definition}).
Then, we define necessary and sufficient conditions for satisfiability of a validity property in synchronous, and partially synchronous environments.

\subsection{Validity of the Crash-Stop Consensus: Formal Definition} \label{subsection:crash_stop_definition}

Let us fix the $f$-resilient crash-stop consensus problem $\mathcal{P}_C$.

We start by defining a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x$ is either $P \in \Psi$ or $\bar{P}$, with $P \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$; on the other hand, $(\bar{P}, \mathit{val}')$ denotes that a \emph{faulty} process $P \in \Psi$ has proposed a value $\mathit{val}' \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.
Finally, $\mathit{pp}.\mathsf{correct}$ returns $\mathit{true}$ if and only if $\mathit{pp}$ is associated with a correct process; otherwise, $\mathit{pp}.\mathsf{correct}$ returns $\mathit{false}$.

An \emph{input configuration} is a tuple $\big[\mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_n \big]$ such that (1) $\mathit{pp}_i$ is a process-proposal pair, for every $i \in [1, n]$, (2) every process-proposal pair is associated with a distinct process which belongs to $\Psi$, and (3) at most $f$ process-proposal pairs refer to faulty processes (i.e., there can exist at most $f$ process-proposal pairs of the format $(\bar{P}, \cdot)$, where $P \in \Psi$).
We denote    by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$.

==> sections/extensions.tex <==
\section{Beyond our Formalism}

\subsection{Extension to External Validity} \label{subsection:external_validity}

\subsection{Extension to Crash-Stop Validity}

==> sections/external_main.tex <==
\section{Extended Formalism: A Brief Introduction} \label{section:extended_formalism_main}

In this section, we briefly introduce an extended version of our formalism to accommodate for blockchain-specific validity properties.
Namely, we make our formalism more expressive by (1) allowing the input ($\mathcal{V}_I$) and output ($\mathcal{V}_O$) spaces to be unknown to processes, and (2) taking into account the ``proposals'' of faulty processes.
The full extended formalism can be found in \Cref{section:extended_formalim_appendix}. \Cref{section:classification_extended,section:blockchain_validity_appendix} are devoted to reestablishing, in the extended formalism, our previous results.

\paragraph{Intuition.}
In the original formalism, processes know the entire input ($\mathcal{V}_I$) and output ($\mathcal{V}_O$) space.
That is, processes are able to ``produce'' any value which belongs to $\mathcal{V}_I$ or $\mathcal{V}_O$.
However, this assumption limits the expressiveness of the formalism as it is impossible to describe a Byzantine consensus problem in which input or output spaces are unknown.
Let us give an example.

Imagine a committee-based blockchain which establishes two roles:
\begin{compactitem}
    \item \emph{Clients} are the users of the blockchain.
    They issue \emph{signed} transactions to the blockchain.
    
    \item \emph{Servers} are the operating nodes of the blockchain.
    Servers receive signed transactions issued by the clients, and solve the Byzantine consensus problem to agree on the exact order the transactions are processed.
\end{compactitem}
The Byzantine consensus problem at the heart of our blockchain satisfies \emph{External Validity}: if a transaction is processed, then it satisfies a predetermined $\mathsf{valid}$ predicate.
Notice that, for example, \emph{Strong Validity} is not suitable in this case, as, if not all correct processes propose the same transaction, \emph{any} transaction (even a ``useless'' one, such as $\bot$) can be decided.
Since servers rarely propose the same transactions, \emph{Strong Validity} would render our system useless a majority of the time.

As servers propose transactions \emph{signed by the clients} and servers do not have access to the private keys of the clients, servers do not know the input space $\mathcal{V}_I$ nor the output space $\mathcal{V}_O$.
% of the Byzantine consensus problem.
Hence, our original formalism is insufficient to describe the Byzantine consensus problem in the core of the aforementioned blockchain.
To address such scenarios, we introduce the extended formalism.

\paragraph{Extended vs. original formalism.}
As highlighted above, the main difference between the two formalisms is that the extended one allows us to specify the ``knowledge level'' of the input and output spaces.
In the extended formalism, a process is able to ``learn'' output values by observing input values.
That is, we define a \emph{discovery function} that specifies which output values are learned given observed input values.
In the committee-based blockchain example, once a server observes signed transactions $\mathit{tx}_1$ and $\mathit{tx}_2$, it learns the following output values: (1) $\mathit{tx}_1$, (2) $\mathit{tx}_2$, (3) $\mathit{tx}_1 || \mathit{tx}_2$, and (4) $\mathit{tx}_2 || \mathit{tx}_1$; we denote by ``$||$'' the concatenation.
% \footnote{We denote by ``$||$'' the concatenation operation.} 

The second difference between the original and the extended formalism is that the extended formalism takes into account the ``proposals'' of Byzantine processes.
Indeed, the original formalism does not allow us to define which values are admissible given the adversary's knowledge of the input space.
Think of the aforementioned example with a blockchain system.
If no process (correct or faulty) obtains a transaction $\mathit{tx}$ from the clients, $\mathit{tx}$ cannot be decided.
However, if \emph{only} a faulty process obtains a transaction $\mathit{tx}$, $\mathit{tx}$ is an admissible decision.
This scenario \emph{can} be expressed by the extended formalism (and not by the original one).



==> sections/lower_bound.tex <==
\section{Lower Bound on Message Complexity}

In this section, we show the quadratic lower bound on message complexity for any partially synchronous algorithm solving the Byzantine consensus problem with a non-trivial validity property.

\begin{definition} [Non-trivial validity property]
Let $\mathit{val}$ be a validity property.
We say that $\mathit{val}$ is \emph{non-trivial} if there does not exist a value $v \in \mathcal{V}$ such that, for every input configuration $i \in \mathcal{I}$, $v \in \mathit{val}(i)$.
\end{definition}

In the rest of the section, we fix a non-trivial validity property $\mathit{val}$ and a partially synchronous distributed algorithm $\mathcal{A}$ that solves the Byzantine consensus problem with $\mathit{val}$.
As $\mathit{val}$ is non-trivial, we have that $n > 3t$ (by \Cref{corollary:trivial_validity}).
In order to prove the lower bound, we show that the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.

First, we define an infinite execution $E_{\mathit{base}}$ in the following manner:
\begin{compactitem}
    \item $\text{GST} = 0$.

    \item We separate all processes into two groups: (1) group $A$, where $|A| = n - t / 2$, and (2) group $B$, where $|B| = t / 2$.
    
    \item All processes from group $A$ are correct.
    
    \item All processes from group $B$ are faulty.
    For each process $P \in B$, $P$ behaves correctly, except that (1) $P$ ignores first $t / 2$ received messages (from other processes), and (2) $P$ does not send any message to any other process in group $B$. 
\end{compactitem}
Let $\mathit{base}$ denote the input configuration which corresponds to $E_{\mathit{base}}$.
Let $\mathit{dec}$ be the value decided in $E_{\mathit{base}}$.
As $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$, $\mathit{dec} \in \mathit{val}(\mathit{base})$.

If correct processes send $\geq (t / 2)^2$ messages in $E_{\mathit{base}}$, the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
In the rest of the proof, by contradiction, we assume that the number of messages sent by correct processes in $E_{\mathit{base}}$ is $< (t / 2)^2$.
We prove that there exists a process $P \in B$ with a valid behavior in which it decides $\mathit{dec}$ without having received any message (from other processes).

\begin{lemma} \label{lemma:p_without_any_message}
There exists a process $P \in B$ such that there exists a valid behavior of $P$ in which (1) $P$ does not receive any message (from other processes), and (2) $P$ decides $\mathit{dec}$.
\end{lemma}
\begin{proof}
Given that correct processes send $< (t / 2)^2$ messages in $E_{\mathit{base}}$, there exists a process $P \in B$ that receives $< t / 2$ messages in $E_{\mathit{base}}$.
Let $S \subset A$ denote the set of processes which send messages to $P$ in $E_{\mathit{base}}$.
Let us now create an infinite execution $E$, which is similar to $E_{\mathit{base}}$:
\begin{compactenum}
    \item We start with $E \gets E_{\mathit{base}}$.
    
    \item For every message which sending was omitted by $P$ in $E_{\mathit{base}}$, (1) the message is sent $E$ (recall that only omitted messages by $P$ are sent to processes in group $B$), and (2) the message is received in $E$ and ignored. 
    
    \item For every message sent to $P$, the sending and receiving events are removed.
\end{compactenum}
For every process $Q \in A \setminus{S}$, the behavior of process $Q$ in $E$ is identical to the one in $E_{\mathit{base}}$.
Hence, $\mathit{dec}$ is decided in $E$.
Moreover, $P$ is correct and it does not receive (from other processes) any message in $E$.
Due to the termination of $\mathcal{A}$, $P$ decides $\mathit{dec}$ in $E$, which concludes the lemma. 
\end{proof}

Finally, we conclude the proof of the lower bound.

\begin{theorem}
The message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
\end{theorem}
\begin{proof}
By \Cref{lemma:p_without_any_message}, there exists a valid behavior of $P$ in which (1) $P$ does not receive any message (from other processes), and (2) $P$ decides $\mathit{dec}$.
As $\mathit{val}$ is a non-trivial validity property, there exists an input configuration $i \in \mathcal{I}$ such that $\mathit{dec} \notin \mathit{val}(i)$.
We fix one such input configuration; let us denote this input configuration by $i$.

We distinguish two cases:
\begin{compactitem}
    \item Let $p \notin i.\mathsf{processes}$.
    In this case, we consider an execution $E_i$ such that (1) $E_i$ corresponds to $i$, and (2) all faulty processes (including $P$) crash immediately (i.e., without taking any computational step).
    In $E_i$, correct processes decide a value $\mathit{dec}_i$ such that $\mathit{dec}_i \neq \mathit{dec}$ (as $\mathit{dec} \notin \mathit{val}(i)$).
    Hence, we can merge execution $E_i$ with the valid behavior of $P$ in which $P$ decides $\mathit{dec}$ without having received any message.
    Thus, disagreement occurs, which contradicts the fact that $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$.
    
    \item Let $p \in i.\mathsf{processes}$.
    We further separate two cases:
    \begin{compactitem}
        \item Let $|i.\mathsf{processes}| > n - t$.
        Let $i^* \in \mathcal{I}$ be an input configuration identical to $i$ except that the process-proposal pair associated with $P$ is removed from $i^*$.
        Note that $|i^*.\mathsf{processes}| \geq n - t$, which means that $i^*$ is a legitimate input configuration.
        Moreover, $P \notin i^*.\mathsf{processes}$ and $i^*.\mathsf{processes} \subset i.\mathsf{processes}$.
        
        Consider an infinite execution $E^*$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (including $P$) crash immediately.
        Let $\mathit{dec}^* \in \mathit{val}(i^*)$ be the value decided in $E^*$.
        
        We prove that $\mathit{dec}^* \in \mathit{val}(i)$.
        By contradiction, suppose that $\mathit{dec}^* \notin \mathit{val}(i)$.
        We build another execution $E_i$ of $\mathcal{A}$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process that decides in $E^*_{\mathit{prefix}}$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, process $P$ is correct and live and have the proposal as specified by $i$.
        \end{compactenum}
        Hence, $E_i$ corresponds to $i$ and the value decided in $E_i$ is $\mathit{dec}^*$.
        Therefore, we reach a contradiction with the fact that $\mathcal{A}$ satisfies $\mathit{val}$, which implies that $\mathit{dec}^* \in \mathit{val}(i)$.
        
        As $\mathit{dec}^* \in \mathit{val}(i)$, $\mathit{dec}^* \neq \mathit{dec}$.
        Therefore, we can merge the execution $E^*$ with the valid behavior of $P$ in which $P$ decides $\mathit{dec}$ without having received any message.
        Thus, disagreement occurs, which contradicts the fact that $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$.
        
        \item Let $|i.\mathsf{processes}| = n - t$.
        In this case, there exists a process $Q$ such that $Q \notin i.\mathsf{processes}$ (as $t > 0$).
        We now build an input configuration similar to $i$:
        \begin{compactenum}
            \item We add $(Q, v)$ to $i^*$, where $v \in \mathcal{V}$ is any value.
        
            \item For every process $P_j \in i.processes \setminus{\{P\}}$, we add $(P_j, \mathit{proposal})$ to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i$.
        \end{compactenum}
        Note that $|i^*.\mathsf{processes}| = n - t$, which means that $i^*$ is a legitimate input configuration.
        Moreover, $P \notin i^*.\mathsf{processes}$.
        
        Consider an infinite execution $E^*$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (including $P$) crash immediately.
        Let $\mathit{dec}^* \in \mathit{val}(i^*)$ be the value decided in $E^*$.
        
        We prove that $\mathit{dec}^* \in \mathit{val}(i)$.
        By contradiction, suppose that $\mathit{dec}^* \notin \mathit{val}(i)$.
        We build another execution $E_i$ of $\mathcal{A}$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process $Q' \neq Q$ that decides in $E^*_{\mathit{prefix}}$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, process $P$ is correct and live and have the proposal as specified by $i$.
            Moreover, process $Q$ crashes.
        \end{compactenum}
        Hence, $E_i$ corresponds to $i$ and the value decided in $E_i$ is $\mathit{dec}^*$.
        Therefore, we reach a contradiction with the fact that $\mathcal{A}$ satisfies $\mathit{val}$, which implies that $\mathit{dec}^* \in \mathit{val}(i)$.
        
        As $\mathit{dec}^* \in \mathit{val}(i)$, $\mathit{dec}^* \neq \mathit{dec}$.
        Therefore, we can merge the execution $E^*$ with the valid behavior of $P$ in which $P$ decides $\mathit{dec}$ without having received any message.
        Thus, disagreement occurs, which contradicts the fact that $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$.
    \end{compactitem}
\end{compactitem}
As the statement of the theorem is satisfied in every possible scenario, the theorem holds.
\end{proof}

\begin{corollary}
Let $\mathit{val}$ be any non-trivial validity property.
Let $\mathcal{A}$ be any partially synchronous distributed algorithm that solves the Byzantine consensus problem with $\mathit{val}$.
The message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
\end{corollary}

==> sections/preliminaries.tex <==
\section{Preliminaries} \label{section:preliminaries}

\paragraph{System model.}
We consider a static system $\Pi = \{P_1, ..., P_n\}$ of $n$ processes among which $t$ processes can be Byzantine; Byzantine processes can behave arbitrarily.
Moreover, $n \geq 2t + 1$.
If a process is Byzantine, the process is \emph{faulty}; otherwise, the process is \emph{correct}.

\paragraph{Byzantine consensus.}
In the Byzantine consensus problem, each process has its \emph{proposal}, and it should eventually \emph{decide}.
We denote by $\mathcal{V}$ the set of value a process can propose and decide.
The Byzantine consensus problem requires the following three properties:
\begin{compactitem}
    \item \emph{Agreement:} No two correct processes decide different values.
    
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Validity}
\end{compactitem}
In the next paragraph, we take a closer look at the validity property of the Byzantine consensus problem.

\paragraph{Validity property.}
A \emph{process-proposal} pair is a pair $(p \in \Pi, \mathit{proposal} \in \mathcal{V})$.
An \emph{input configuration} is a tuple $(\mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_x)$, where (1) $\mathit{pp}_i$ is a process-proposal, for every $i \in [1, x]$, (2) every process-proposal pair concerns a different process (i.e., there does not exist $\mathit{pp} = (p, v)$ and $\mathit{pp}' = (p, v')$ in the input configuration), and (3) $x \geq n - t$. 
We denote by $\mathcal{I}$ the set of all possible input configurations.

Finally, we define a validity property $\mathit{val}$ as a function $\mathcal{I} \to 2^{\mathcal{V}}$ such that, for every $\mathit{input} \in \mathcal{I}$, $\mathit{val}(\mathit{input}) \neq \emptyset$.
Intuitively, if $\mathit{val}(\mathit{input})$ denotes the set of values that can be decided if correct processes propose the values specified by $\mathit{input}$.
For example, let us consider the strong validity property which states that a correct process decides a value proposed by a correct process.
The following captures this property:
\begin{equation*}
    \forall v \in \mathcal{V}, \forall \mathit{input} \in \mathcal{I}: v \in \mathit{val}(\mathit{input}) \iff \exists \text{ process-proposal } (p, v') \in \mathit{input} \text{ such that } v' = v.
\end{equation*}
